Iterative Judgment Aggregation

Judgment aggregation problems form a class of collective decision-making problems represented in an abstract way, subsuming some well known problems such as voting. A collective decision can be reached in many ways, but a direct one-step aggregation of individual decisions is arguably most studied. Another way to reach collective decisions is by iterative consensus building -- allowing each decision-maker to change their individual decision in response to the choices of the other agents until a consensus is reached. Iterative consensus building has so far only been studied for voting problems. Here we propose an iterative judgment aggregation algorithm, based on movements in an undirected graph, and we study for which instances it terminates with a consensus. We also compare the computational complexity of our iterative procedure with that of related judgment aggregation operators.

==> ecai-6-properties.tex <==
\section{Properties of Consensus}\label{sec:properties}

\new{In this section, we compare the output and performance of our deliberation procedure to those of standard distance-based judgment aggregation rules.
We first discuss the ``quality'' of the consensual decision. Then, we look at the computational complexity of the procedure.}


\subsection{Consensus Quality}

Distance-based judgment aggregation~\cite{MillerOsherson08,thesis,TARK11,JamrogaS13} combines an algebraic aggregation function $\star$ with a distance function $d$ (not necessarily a path distance in some agenda graph) in order to select the collective opinion that is closest to the given profile.
%Typically, $\star \in \{\sum, \max\}$
Given $\Pf\in \Dmc^n$, the distance-based aggregation function $F^{d,\star}: \Dmc^n \rightarrow 2^{\Dmc}\setminus \emptyset$  is defined as
$$F^{d,\star} (\Pf) = \argmin{\Js \in \Dmc}\;\; \star(d(\Pf[1], \Js), \ldots, d(\Pf[n], \Js)).$$
Natural questions to ask are:
%
\begin{itemize}
\item How does \alg perform in comparison to $F^{d,\Sigma}$ when $d$ is a path distance in an agenda graph?
\item How do the collective judgments $F^{d,\Sigma} (\Pf^0)$ compare to the consensus judgment reached by \alg for a given starting profile $\Pf^0$?
\end{itemize}
%
The questions cannot be fully explored within the scope of this paper. However, we establish some initial properties below.

\putaway{
  \begin{proposition}It is not always the case that, for a $1$-connected   $\Pf^0 \in \Dmc^n$,   if $F^{d,\Sigma} (\Pf^0) = \Js$, then $\alg$ will reach $\Pf$ with $\{ \Pf\} = \{\Js\}$.
  \end{proposition}
  \begin{proof} Consider the $\A$ and $\Ct$ with   $\gag$ in Figure~\ref{fig:cycle} and the profile $\Pf^0 \in \Dmc^n$, $\Pf^0 = \langle \Js_1, \Js_2, \Js_3, \Js_4 \rangle$. The \alg will not terminate with a consensus for this  $\Pf^0$, but $F^{d,\Sigma} (\Pf^0) = \Js$.
  \end{proof}
}% end-putaway

A property generally deemed desirable in judgment aggregation is that of \emph{propositional unanimity}~\cite{TARK11,thesis,GrandiEndriss13}. Propositional unanimity requires that, if every agent in profile $\Pf$ has the same value for some issue $\ai \in \A$, then the same value for $\ai \in \A$ shows up either in at least one of the judgments in $F^{d, \star}$ (weak unanimity) or in all of the judgments in $F^{d, \star}$ (strong unanimity). It is interesting to note that the most popular distance based judgment aggregation rule $F^{d_h, \Sigma}$ (\ie the one based on the sum of Hamming distances) does not satisfy even the weak version of the property~\cite{ADT09}. The same applies to $F^{d_m, \Sigma}$ and $F^{d_c, \Sigma}$~\cite{LangPSTV15}. In this respect, consensus behaves better.

\new{
\begin{proposition}\label{prop:unanimity-H}
If \alg terminates with a consensus on $\gag^h$, then the consensus satisfies weak unanimity with respect to the initial profile $\Pf^0$.
\end{proposition}
%
\begin{proof}
%Note that, for $\gag^h$ and $\gag^m$, if judgment $\Js'$ is between judgments $\Js$ and $\Js''$,  then vertex $\Js'$ is on the shortest path between vertices $\Js$ and $\Js''$ in the graph. For $\gag^h$, the implication actually goes in both directions.
Note that, for $\gag^h$, judgment $\Js'$ is between judgments $\Js$ and $\Js''$ iff vertex $\Js'$ is on the shortest path between vertices $\Js$ and $\Js''$ in the graph.
Consequently, if all the agents in $\Pf^0$ give the same truth-value on an issue, then $\CH(\Pf^0)$ cannot contain judgments that assign different truth-value to this issue.
\end{proof}

The same is not the case for $\gag^m$. 

\begin{proposition}\label{prop:unanimity-M}
There is an initial profile $\Pf^0$ such that \alg terminates with a consensus on $\gag^m$, and the consensus does not satisfy weak unanimity with respect to $\Pf^0$.
\end{proposition}
%
\begin{proof}
As a counter-example consider   Example~\ref{ex:doctrinal} and Graph $b$ in Figure~\ref{fig:doctrinalexample}. The vertex $(1,1,1)$ is between vertices $(0,1,0)$ and $(1,0,0)$, but the judgment $(1,1,1)$ is not between judgments $(0,1,0)$ and $(1,0,0)$. Thus the agents can move from $(0,1,0)$ and $(1,0,0)$ to  $(1,1,1)$  thus violating propositional unanimity on the last agenda issue.
\end{proof}

A big advantage of one-shot distance-based aggregation $F^{d,\Sigma}$ is that it produces output (a winner or winners) on any profile $\Pf^0$, while our \alg is more restricted in this respect. As we have seen, a necessary condition for successful termination of \alg is that $\Pf^0$ is 1-connected. Sufficient conditions are even more restrictive.
Still, Proposition~\ref{prop:unanimity-H} demonstrates that, when \alg reaches a consensus, it is structurally ``better behaved'' then a distance-based judgment aggregation rule for the most popular approach based on the sum of Hamming distances.
In the next subsection we show that \alg is also ``better behaved'' in the sense of computational complexity.
}% end-new

\subsection{Complexity of Reaching Consensus}

\new{An important drawback of distance-based judgment aggregation is the computational complexity of producing the output, \ie the winning judgment or judgments.
The winner determination problem for $F^{d_h,\Sigma}$ is known to be $\Theta^p_2$-complete~\cite{EndrissGP12}, and the result extends to most other distances $d$ and aggregation functions $\ast$~\cite{JamrogaS13}.
How does it work for the deliberation procedure formalized with \alg?}

We have shown that the algorithm reaches consensus for an odd number $n>3$ of agents on $1$-connected, not equidistant profiles. How costly is it to reach the consensus? On $\gag^c$, it is evident that \alg performs well, but the resulting consensuses are not very exciting.  For the $\gag^m$ graph, the consensus-friendly attitude does not earn much in terms of computational complexity, when compared to  $F^{d_m,\Sigma}$.
For each $\Pf[i]$, we need to find every $\Js \in \Dmc$ s.t. there is no rational judgment between $\Pf[i]$ and $\Js$. It is not difficult to show, by a reduction to coSAT, that checking whether there is no rational judgment between two rational judgments is a coNP-complete problem.
This has to be repeated for multiple candidate judgments to compute the set \moves, and on top of that with every iteration of the algorithm. As a consequence, we get the following.

\begin{theorem}
For $\gag^m$, determining the winners of a single iteration of \alg is coNP-hard.
\end{theorem}

We conjecture that the problem is actually $\Theta_2^P$-complete.
\new{Note that the hardness result is not really due to the deliberation procedure, but rather due to the inherent complexity of computing $d_m$, which requires to determine (non)existence of particular rational judgments, \ie to solve the Boolean co-satisfiability problem.

In contrast, the Hamming distance $d_h$ can be always computed efficiently. Consequently, when \alg reaches a consensus on $\gag^h$, it is also ``better behaved" computationally than the distance-based judgment aggregation rule $F^{d_h,\Sigma}$. We demonstrate it formally below.}

\begin{proposition}
For $\gag^h$, a single iteration of \alg runs in deterministic polynomial time.
\end{proposition}
%
\begin{proof}
Follows from the fact that the set \moves can be constructed by checking at most ${|\A|}$ candidate judgments.
\end{proof}

By Corollary~\ref{lem:mcyc}, if the $\CH(\Pf^0)$ induced subgraph of $\gag^h$ has no cycles, then $\CH(\Pf)$ is strictly shrinking with each non-terminating step $t$. In consequence, if \alg reaches consensus for such $\Pf^0$, then it does so in polynomially many steps.
However, in case of cycles in the $\CH(\Pf^0)$ induced graph  in $\gag^h$, the algorithm may run into such a cycle and take some time until the agents ``stray'' from the loop. When it happens, any judgment occurring on the loop can be the consensus.
%Assume the probability of all the agents staying on the cycle in one round to be $p$. Then, the expected number of iterations until they stray from the cycle is $\sum_{i=1}^\infty i\cdot p^{i-1}\cdot (1-p) = ????$
Using this observation, we propose the following modification of \alg.

\para{\algtwo:} Same as \alg, \new{only it stops the deliberation when  $\{\Pf_t\}= \{\Pf_{t'}\}$ for some $t>t'$}, and nondeterministically chooses one $\Js\in\{\Pf\}$ as the consensus, producing in the next step $\Pf_{t+1}$ with $\{\Pf_{t+1}\} = \{ \Js\}$.

\new{Unlike \alg, \algtwo avoids looping and waiting until two or more agents ``move'' in the same direction.
It also avoids infinite loops in the case of profiles with evenly many agents.
%because as soon as  an even number of the agents  split into two same size groups, one choosing  $\Js$ and the other an adjacent $\Js'$, the algorithm will terminate and one of $\Js$ and $\Js'$ will be  chosen as a consensus at random.
On the other hand, \algtwo is no longer decentralised, which is a clear disadvantage.
We suggest that it can be treated as a technical variant of \alg that potentially reduces its running time by employing a trusted third party which simulates probabilistic convergence of the profile in \alg by one-step nondeterministic choice in \algtwo.}
The following formal results, which are straightforward consequences of our analysis above, justify the suggestion.

\begin{theorem}
Consider $\gag^h$ and $N$ such that $|N|$ is odd and larger than 3. 
\new{If \alg can reach consensus with $\Js$ then also \algtwo can reach consensus with $\Js$.}
\end{theorem}

\begin{theorem}
Consider $\gag^h$ and $N$ such that $|N|$ is odd and larger than 3. Moreover, let $\Pf^0 \in \Dmc^n$ be 1-connected and not equidistant. 
\algtwo reaches consensus from $\Pf^0$ on $\gag^h$ in deterministic polynomial time.
\end{theorem}

% WE ACTUALLY DON'T WANT TO DISCUSS THE FOLLOWING:
%We here discuss how computationally difficult it is to determine whether the algorithm will terminate for a given $\Pf^0$.
%For the Hamming distance, checking whether $\Pf^0 \in \Dmc^n$ is $1$-connected can be done in polynomial time with respect to  $n \times |\A|$. Namely,  every judgment in $\Dm$ has exactly $|\A |$ judgments at Hamming distance 1. For each agent $i$ we need to check which of the judgments at Hamming distance 1 from $\Js^0_i$ are rational. Note that for $d_h$,  when  $\Pf^0 \in \Dmc^n$ is $1$-connected, the consensus can be found in polynomial time with respect to  $n \times |\A|$.
%For the distance $d_m$, by definition, every profile is  $1$-connected. However, the problem of finding the consensus, \ie running the algorithm, is no longer polynomial, because determining the possible moves for an agent can no longer be done in polynomial time. Namely, Since $n$ and $|\A|$ are fixed, finding a path between two rational judgments is also in  {\sc NP}: guessing a path and checking that each judgment in it is rational. Thus  determining the possible moves for an agent  would require no less than $n-1$ calls to an {\sc NP}-oracle, one for each  agent in the profile.

Lastly, let us observe that checking whether $\Pf^0$ is equidistant can be done in linear time of the number of agents.
For a graph $G$, determining if  it has a simple cycle of size $k$, for $k$ fixed,  is a  polynomial time problem over the size of $G$ \cite{Alon:1997}, however we do not generate the full $\gag$ when (or before) we run the deliberation algorithm.


==> ecai-8-conclusions.tex <==
\section{Conclusions}\label{sec:sum}

We propose a decentralised  algorithm for deliberation on judgment aggregation problems.  Since judgment aggregation is an abstract framework, it allows for other social choice aggregation problems, such as voting, to be represented in it, see \eg  \cite{aaai} for a recent overview. We study the termination conditions for this algorithm and its complexity properties.

For reaching a consensus our algorithm exploits the topology of a graph - all available judgments that the agents can chose from are vertices in a graph and the algorithm models moves along adjacent judgments in the graph.  We define three intuitive graphs that can be constructed for a set of rational judgments $\Dmc$: the complete, the Hamming and the model agenda graph $\gag^c$, $\gag^h$, and $\gag^m$ respectively.  We show that our algorithm always terminates for an odd number of agents on the graph $\gag^c$, but it necessarily selects one of the judgments proposed in the first round of deliberations. For the graphs  $\gag^h$  and $\gag^m$ we show a class of profiles for which the algorithm terminates with a consensus and a class of profiles for which it does not terminate with a consensus.

%If the profile is equidistant, namely each agent has  chosen judgments with the same path distance to each of the judgments of the other agents, then the \alg does not terminate with a consensus.
If the agents initially chose judgments such that the convex hull of the profile of these judgments  induces a subgraph of $\gag^h$,  or  $\gag^m$ in which each vertex has a degree of at most 2, then our algorithm probabilistically terminates with a consensus for an odd number of (more than 3) agents.

The list of  profiles we give here,  for which  \alg terminates with a consensus,  is clearly not exhaustive. For example, it is easy to show that, for an odd number of agents,  \alg terminates with a consensus if the $\CH(\Pf^0)$ induced subgraph  of $\gag^h$,  or  $\gag^m$, is such that it contains only $k$-cycles, where $k= 2\cdot mx_d(\Pf^0) +1$. This is because for such profiles there exists at least one pair of antipodal judgments with degree no more than 2 who will have a nonempty set \moves. %This means that the starting profile $\Pf^0$ would be allowed to only have cycles of the same size. The doctrinal paradox profile has a convex hull whose induced subgraph of $\gag^h$ satisfies this condition as it can be directly observed in Figure~\ref{fig:hull}. 
An immediate direction for future work is to strengthen our results with other classes of consensus terminating agenda graph topologies, particularly those corresponding to profiles on the preference agenda (and transitivity constraints).

A step of our algorithm implements  a judgment profile transformation function of the type defined in \cite{List2011}. List \cite{List2011} gives an impossibility characterisation of such functions. Our function ``escapes" this impossibility result by not satisfying  the independence property  on all agenda graphs and the universal domain on $\gag^h$.

While  $\gag^c$,   and $\gag^m$ satisfy the necessary conditions for termination of \alg for any $\A$ and $\Ct$, this is not the case with $\gag^h$, which is why the transformation function fails to satisfy universal domain on $\gag^h$. On  $\gag^h$, sometimes all the adjacent judgments to a rational judgment $\Js$ are not rational and thus not allowed to move to. In our future work we aim to explore modifications of the algorithm allowing the agents to make ``longer" moves, \ie to ``jump over" a vertex that is not a rational judgment.

In Section~\ref{sec:properties} we gave two results with respect to the quality of the  consensus reached by \alg with respect to the widely used distance-based aggregation function $F^{d_h, \Sigma}$.  This function $F^{d_h, \Sigma}$ is also known as the median aggregation rule and it is widely used in many domains, \eg  generalises the Kemeny voting rule, see \cite{ADT2013},  and for measuring dissimilarity between concepts in ontologies \cite{DistelAB14}. We merely scratched the surface of this consensus quality analysis and this line of research merits further attention.

Lastly, a more longterm goal for our future work is to explore versions of deliberation on an agenda graph where the agents do not try to move to reduce the path distance to all of the other agents, but only to their neighbours in a given social network, or as in \cite{Goel2012}, to two randomly selected two agents.

